Robots Influencing Humans to Reveal their Goals during Collaboration and Competition

We propose a unified strategy for fast goal inference in human-robot interaction. The core idea is to drive the human toward Critical Decision Points (CDPs)-states where competing human strategies prescribe different next actions and thus maximally reveal the goal. We formalise CDPs using a goal-conditioned policy divergence measure and incorporate them into a Receding-Horizon Planner that explores future action sequences while optimizing a cost function balancing task progress and information gain. We evaluate this approach in both a collaborative, fully observable cooking task and a competitive, partially observable hide-and-seek game, each in simulation and on real robots. In both scenarios, our method infers human goals more accurately and earlier than baseline strategies.

==> Sections/Old/CDP.tex <==
\section{Reasoning about Informative Cues in the State Space}

\subsection{Problem Definition}

We consider a robot working alongside a person in a shared environment and aim to enable the robot to infer the person’s high-level strategy.  We model a human strategy as a policy $\pi$ that maps each full environment state $s=(s_w,s_h,s_r)$ to an action, where $s_w$ is a discrete world description (e.g., an occupancy map or object configuration), $s_h$ is the human’s state, and $s_r$ is the robot’s state.  The robot always has full access to $s_w$ and $s_r$, but it perceives $s_h$ only through its (possibly noisy or partial) observations of the human’s behavior.  To capture a range of plausible behaviors, the robot is equipped with a policy bank, denoted as \( \mathcal{P} = \{\pi_1, \dots, \pi_n\} \). This policy bank may include various strategies for different scenarios. For instance, in a competitive navigation task, it could feature different hiding strategies. In a collaborative cooking task, the policy bank would encompass strategies for completing various recipes that the human and robot could prepare together.  During execution, the robot maintains a belief, a probability distribution over $\mathcal{P}$, and treats the most probable policy $\hat{\pi}_h$ as its current estimate of the human’s true strategy.  We assume the human’s actual policy, $\pi_h^*$, remains fixed throughout a single interaction.

The exact formulation applies to both competitive and collaborative scenarios, with a few extensions specific to the collaborative case. In the collaborative scenario, we assume that both agents share and fully observe the state $s$ and they record the entire history of actions $\mathcal{H}$ taken so far.  We further assume that once an atomic action occurs, it does not repeat. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/CDP.pdf}
    \caption{\textbf{Critical Decision Point Computation}. For every policy of the human in the policy bank, we compute what states in the environment produce the most divergent actions. For instance, if there were four reasonable policies the human could be following, at $s_1$, all four of them produce different actions, making $s_1$ a Critical Decision Point (as compared to $s_2$ and $s_3$ where most policies predict the same action). }
    \vspace{-1em}
    \label{fig:CDP}
\end{figure}

\subsection{Critical Decision Points}

The primary insight of our work is that there are states in the environment where observing a human take an action can reveal important information about their high-level strategy. We refer to those states as Critical Decision Points ($S_{crit}$), for which the divergence in the human's potential actions (as per the policy bank $\mathcal{P}$) is maximized. 
Mathematically, let the environment state $s_w$ be represented by a grid, with each grid cell having semantic information about that specific location in the world. For example, if the grid is 2-dimensional, then each cell can contain occupancy information. If the grid is higher-dimensional, then more or alternative semantic features about the environment can be included in the representation. Then, for each possible grid cell $s_w^{(i,j)}$ in the environment state, we compute ($S_{crit}$) as:
\begin{align}
\label{eq: cdp}
        \hspace{-1em} 
        S_{crit} = \{s_w^{(i,j)} \, |\, strategy\_div(\mathcal{P}, s^{(i,j)}) > \theta\},
\end{align}

\noindent
where $s^{(i,j)}$ represents the full state of the world with the human agent being located at the grid cell $s_w^{(i,j)}$, $strategy\_div(\mathcal{P}, s^{(i,j)})$ measures the divergence in the strategies of the policy bank $\mathcal{P}$, and $\theta$ is a threshold for the divergence. Depending on the task, $strategy\_div()$ can be calculated as the count of the number of actions differing at a given state or quantified as some similarity measure of the next states.  
The central hypothesis of our work is that at Critical Decision Points, the human's actions will be more revealing about their strategy to an observing robot than other states in the environment, as shown in Fig. \ref{fig:CDP}. 

\subsection{Informative States}

The original formulation of $S_{crit}$ (see Eq. \ref{eq: cdp}) required exhaustive offline computation of policy divergence for every state across the entire state space. Such exhaustive computation is infeasible in realistic, long-horizon collaborative tasks with large state spaces. Moreover, in long-horizon collaborative tasks, the criticality of a state is affected by the action sequence taken during the interaction to reach the state. Therefore, it was essential to define Informative States that build upon the definition of a CDP by considering not only the current state but also the action history leading to that state. We define:
\begin{align}
\label{eq: informative_state}
    S_{inform} = \{ s \in S \mid strategy\_div(\mathcal{P}, s, \mathcal{H}^{0:t-1}) > \theta \},
\end{align}


where $strategy\_div(\mathcal{P}, s, \mathcal{H}^{0:t-1})$ measures the divergence of the policies in the policy bank $\mathcal{P}$ at state $s^t$, given the shared action history $\mathcal{H}_a^{0:t-1}$. In effect, this definition of Informative States $S_{inform}$ allows for a dynamic, history-informed estimation of Critical Decision Points (CDPs), efficiently evaluating policy divergence online as the interaction progresses.


==> Sections/Old/Influencing.tex <==
\section{Influencing Humans to Reveal their Goals}

% \subsection{Using Receding Horizon Planning to Influence Humans} 

We develop a method for the robot to reduce the uncertainty of its belief over the human's current strategy, given the set of reasonable human policies in the policy bank $\mathcal{P}$, in both competitive and collaborative tasks. We frame the above problem as a discrete-time planning problem, which we solve using a Receding Horizon Planning (RHP) approach \cite{ma2006receding}. RHP takes inspiration from Model Predictive Control  \cite{garcia1989model} but concerns discrete decision-making rather than continuous control. Generally, to perform RHP, an agent iteratively solves a planning problem over a receding horizon, considering possible future actions by expanding a search tree. After planning on a given time step, the first action leading to the best possible outcome is executed, the horizon window moves forward, and planning is performed again for the next possible futures.

\subsection{Influencing Humans to Reveal their Goal in a Competitive Task at CDPs}
\label{sec: influence_competitive}

\input{Sections/Algorithms/competitive_algo}

\begin{figure}[t!p]
    \centering
    \includegraphics[width=\linewidth]{Figures/MPC_obstacles.pdf}
    \caption{\textbf{Example RHP tree rollout for influencing the robot in a competitive hide and seek game: } The green and the blue agent are playing a hide-and-seek game, where the green agent (the seeker) is trying to influence the blue agent (the hider) to a Critical Decision Point (the red cell) using RHP to infer its policy and therefore catch it faster. The brick walls represent obstacles. The green agent imagines all possible future actions, assuming the blue agent follows a fixed policy, and selects the most optimal action in the next timestep to lead to the most favorable outcome at horizon $\mathcal{D}=t_4$. The black arrow at $t_1$ represents the underlying strategy. Both agents' fields of view are restricted to all the cells in the direction they face. At $t_2$, when the blue agent detects the green agent, it abandons its underlying strategy at  $t_3$ to perform an evasive maneuver, then resumes its original path once out of the green’s field of view at $t_4$. This allows the green agent to observe the blue agent's underlying policy at a critical decision point at $t_3$ without being observed, and ultimately catch it in $t_4$. Note that the green arrow denotes the optimal next action for the green agent. After rolling out all possible futures, the green agent determines its optimal sequence of actions to be $a_2 \rightarrow a_1 \rightarrow a_1$ (highlighted in white). Since the green agent performs RHP, it takes the first action $a_2$ from the sequence and constructs the tree from the next state. }
    \vspace{-1em}
    \label{fig:mpc}
\end{figure}


Alg. \ref{algorithm} summarizes our approach for a robot to influence a human towards Critical Decision Points. 
At a given time $t$, the robot rolls out all possible future actions that can be taken by the human per the policy bank $\mathcal{P}$ along with its own responses to the human's possible actions. These steps are repeated to grow the search tree to a certain horizon $\mathcal{D}$. For every leaf node in the tree that results from the human acting according to a policy $\pi_i$, the robot computes a cost $\mathcal{C}_{\pi_i}(s^t)$ that describes how good that specific future is based on 1) the
distance between the projected human position at time $t + \mathcal{D}$ and the closest Critical Decision Point ($s_{crit}$), and 2) the satisfaction of other task-related objectives:
\begin{align}
    \mathcal{C}_{\pi_i}(s^t) = (\lambda_{1}dist(s_h^{t+\mathcal{D}}, s_{crit}) + \lambda_{2}C_{task})\dfrac{1}{bel(\pi_{i}^t)}
    \label{eq:rhp_cost}
\end{align}
where $dist(s_h^{t+\mathcal{D}}, s_{crit})$ is the shortest path between the human and the closest Critical Decision Point $\mathcal{D}$ steps in the future when the human acts according to $\pi_i$ and the robot takes corresponding actions, $C_{task}$ is a task-specific cost function,  and $\lambda_{1}, \lambda_{2}$ are weights to balance the two objectives. The cost $\mathcal{C}$ is scaled by the likelihood of the human policy $bel(\pi_i^t)$, such that less likely policies result in higher cost. We compute $bel(\pi_i^t)$ recursively over time with a Bayesian update, similar to a Bayes Filter \cite{thrun2006probalistic} with an identity transition function as we assume that the human does not change the actual underlying strategy $\pi_h$ during an interaction:
\begin{equation}
\begin{aligned}
    bel(\pi_i^t) &= P(\pi_i^t|s^1 \ldots s^t) \propto P(s^t|\pi_i)\, bel(\pi_i^{t-1})\\ 
    \implies bel(\pi_i^t) &= P(s^t|\pi_i)\, bel(\pi_i^{t-1})
    \label{eq:belief}
\end{aligned}
\end{equation}
where % $bel(\pi_h^t)$ is the posterior probability of a human's policy based on the states observed up until time $t$ and 
$bel(\pi_i^{t-1})$ is the prior belief at time $t-1$, and the probability of a state given a human policy, $P(s^t|\pi_i)$, is computed empirically based on state visitation frequencies of the human when they are following the given policy. %, $bel(\pi_h^{t-1}|s_h)$ is the prior belief over all possible policies, and $P(s_h)$ is the normalization factor.

Finally, the robot selects its best response action $a_r^*$ at time $t$ as the action that minimizes the cost function $\mathcal{C}_{\pi_i}(s^t)$ for all possible $\pi_i \in \mathcal{P}$ over the horizon $\mathcal{D}$. This allows it to influence the human toward Critical Decision Points, because the cost is dependent on where the human ends up after $\mathcal{D}$ steps in the future. 

\subsection{Influencing Humans to Reveal their Goal in a Collaborative Task at Informative States}

\input{Sections/Algorithms/collaborative_algo}

Explicitly inducing a human towards CDPs in a collaboration task as described in Sec. \ref{sec: influence_competitive} can be risky. First, when attempting to do so, the robot could take an action that is detrimental to the collaborative task because it does not know for certain what the human's goal is. Second, because the actions of the human and the robot are intertwined, it is possible for the robot to act from a CDP in a way that negatively affects its understanding of the human's true goal. 
As a result, in this work, we do not attempt to enforce that the human reaches an Informative State via the robot's actions, but instead enable the robot to act in a way that maximizes the chance of success while reducing uncertainty about the human's goal.

Alg. \ref{algo} describes our Receding Horizon Planning (RHP) approach for selecting the robot's action at a given timestep, such that the robot could influence the human to take more distinguishing actions at Informative States. First, we expand an RHP tree with the current interaction sequence (i.e., the history of actions leading up to the last action taken by the human) as its root. To do this recursively, we iterate through every leaf node in the tree, which is a sequence of possible future actions both agents can take from the root node of the tree  (line 6). Then, for each valid action from the corresponding state, we execute that action and add the resultant state as a child node to the selected leaf node (lines 7-11). We continue this process until we reach depth $\mathcal{D}$. Then, we observe the history of actions taken only by the human (line 15), and use this to calculate the cost for every leaf node according to Eq. \ref{eq: cost} (lines 16-17). Finally, we return the first action leading to the leaf node with the lowest cost.

We steer the robot in the collaboration towards taking actions that are 1) unlikely to be detrimental to achieving the human's goal and 2) unlikely to significantly alter the robot's belief about human goals. 

For the first consideration, we induce the robot to take general actions that are common for reaching multiple goals. Intuitively, as the task progresses, the robot’s tendency to act generically reduces the availability of general actions for the human, effectively pushing them to act in ways that clarify their true goal.
We formalize this via a generality score $G(\mathcal{F}^t)$, where $\mathcal{F}^t$ is a sequence of future actions taken from the state $s^t$. For a given sequence $\mathcal{F}^t$, the score is computed by estimating how often the policies in the bank $\mathcal{P}$ would result in the same sequence of actions as in $\mathcal{F}^t$.

For the second consideration regarding the belief about human goals, we calculate a similarity measure that enables the robot to identify actions that minimize changes to this belief. We compute this similarity measure as the similarity of actions available from each state in the state space. 
This similarity measure takes into account the action history of an interaction up to state $s^t$, which we refer to as $\mathcal{H}^{0:t-1}$, and a possible sequence of future actions $\mathcal{F}^t$ from $s^t$:
\begin{align}
\label{eq: similarity}
    similarity(bel(\mathcal{H}^{0:t-1}),bel(\mathcal{F}^t))
\end{align}
where $bel(\cdot)$ corresponds to the likelihood over possible human goals induced by the policies in $\mathcal{P}$ given the input sequence, either past or future actions. We calculate similarity using cosine similarity in this work; however, other measures, such as Wasserstein distance, could also be used as an alternative. Intuitively, this similarity measure acts as a proxy for $strategy\_div$ from Eq. \ref{eq: informative_state} in large state spaces because a state will likely be an Informative State if it permits many dissimilar actions.

Taking both considerations together, the robot ends up acting by choosing a branch of the RHP tree that minimizes the cost:
\begin{align}
\label{eq: cost}
    C = -similarity(bel(\mathcal{H}^{0:t-1}),bel(\mathcal{F}^t)) - \lambda*G(\mathcal{F}^t)
\end{align}
This cost is implemented in lines 16-17 of Alg. \ref{algo}, where the input sequence of past actions is computed in line 15, and the future possible actions are computed in lines 3 to 14.

\begin{figure}[t]
    \centering  
    % \includegraphics[width=\linewidth]{Figures/rhp_tree.png}
    \includegraphics[width=\linewidth]{Figures/rhp_tree_1.png}
    \caption{\textbf{Selecting actions to infer the human's goal at an Informative State for a human-robot collaborative cooking task:} A Receding Horizon Planning (RHP) tree of all possible actions the human and the robot can take in a turn-based interaction is expanded, where the human takes the first turn. The circles correspond to states, and the arrows correspond to the possible action sequences taken at a given time step. The color of the circles indicates the possible goals that can be reached from a given state. The belief distribution is shown at steps $t_0$ and $t_2$, as the robot updates its belief over the human's goals when a human action is observed.  The green arrows show the actions that would optimize the cost function in Eq. \ref{eq: cost}. See the text for more details. 
}
% \vspace{-2em}
    \label{fig:cdp_sequence}
\end{figure}


Figure \ref{fig:cdp_sequence} illustrates how our proposed approach works. A tree of all possible actions the human and the robot can take in a turn-based interaction is expanded, where the human takes the first turn. After $t_0$, the robot is already biased towards either the parfait or oatmeal being the human's goal, so it chooses a more general overlapping action (gathering a spoon) to influence the human into an  Informative State, which would be either gathering the salt or the sugar. At the Informative State ($t_2$), the human would gather sugar, which disambiguates between the two most likely goals, leading the robot to update its belief and confirm the parfait as the goal. The robot can then align its actions with the actual objective, which in $t_3$ is gathering the glass. The green arrow shows the path that minimizes the cost. The robot would take the first action on this path, observe the environment, and reconstruct the tree at the next step.


 
